A state redistribution algorithm for finite volume schemes on cut cell meshes

In this paper we develop a new technique, called \textit{state redistribution}, that allows the use of explicit time stepping when approximating solutions to hyperbolic conservation laws on embedded boundary grids. State redistribution is a postprocessing technique applied after each time step or stage of the base finite volume scheme, using a time step that is proportional to the volume of the full cells. The idea is to stabilize the cut cells by temporarily merging them into larger, possibly overlapping neighborhoods, then replacing the cut cell values with a stabilized value that maintains conservation and accuracy. We present examples of state redistribution using two base schemes: MUSCL and a second order Method of Lines finite volume scheme. State redistribution is used to compute solutions to several standard test problems in gas dynamics on cut cell meshes, with both smooth and discontinuous solutions. We show that our method does not reduce the accuracy of the base scheme and that it successfully captures shocks in a non-oscillatory manner.

==> conservation.tex <==
\subsection{Conservation}\label{sec:cons}
From the first, second, and third order state redistribution algorithms in Section \ref{sec:srdAlg}, the mass of the numerical solution at $t^{n+1}$ is
\begin{equation}\label{eq:total_mass}
\mathcal{M}^{n+1} = \sum^N_{i=1} h_i U^{n+1}_i.
\end{equation}
From the definition of $U^{n+1}_i$ in \eqref{eq:final_update}, the above can also be written as a sum of mass contributions from each merging neighborhood, i.e.,
\begin{equation}\label{eq:total_mass2}
\mathcal{M}^{n+1} = \sum^N_{i=1} \hat{\mathcal{M}}_i,
\end{equation}
where the mass contribution of merging neighborhood $i$ is
\begin{equation}\label{eq:mi}
\hat{\mathcal{M}}_i = \sum_{k \in M_i}\frac{1}{N_k} \int_{\Omega_k}\hat q_i(x) ~d\Omega_k,
\end{equation}
and $\hat q_i(x)$ is the neighborhood's reconstruction.  From \eqref{eq:qi}, \eqref{eq:mi} becomes
\begin{equation}\label{eq:mi1}
\hat{\mathcal{M}}_i = \hat Q_i \hat V_i.
\end{equation}
% \subsection{First order algorithm}
% When $\hat q_i(x)$ is constant, i.e. $\hat q_i(x) = \hat Q_i$ by \eqref{eq:q_avg} and Step 2 in Section \ref{sec:first_order}, \eqref{eq:mi} becomes 
% Substituting \eqref{eq:mi} into \eqref{eq:total_mass2}, we have
% \begin{equation}\label{eq:mi1}
% \hat{\mathcal{M}}_i = \hat Q_i \hat V_i.
% \end{equation}
% by \eqref{eq:q_avg} in the first order algorithm, by \eqref{eq:pq2} in the second order algorithm, and by \eqref{eq:q2} in the third order algorithm.
From \eqref{eq:modV} and \eqref{eq:q_avg1}, \eqref{eq:mi1} becomes
\begin{equation}\label{eq:mi2}
\hat{\mathcal{M}}_i = \sum^{M_i}_{k = m_i}\frac{h_k}{N_k} \hat U_{k}.
\end{equation}
Substituting \eqref{eq:mi2} into \eqref{eq:total_mass2}, the mass at $t^{n+1}$ is
$$
\mathcal{M}^{n+1} = \sum^{N}_{i=1} h_i \hat U_i,
$$
which shows that $\mathcal{M}^{n+1}  = \mathcal{M}^{n} $.

